On Minc's sheltered middle path

This paper shows that a construction, which was introduced by Piotr Minc in connection with a problem that came from Helly type theorems and that allows to replace three PL-arcs with a "sheltered middle path", can in the case of general (non-PL) paths result in the topologist's sine curve.

==> pseudo.tex <==
 # pltyp := .. ;        #  
 # plvariante := .. ;   #
 # SELECT " ... ";      #
 # .. SIZE .. ;         #
 # pens(  1) := .. ;    #
 # pens(  2) := .. ;    #
 # ...                  #
 # pens(256) := .. ;    #
 # initialise;          #
   0.00000 UPTO   1.00000 WINDOW   0.00000 UPTO   1.00000;
 PEN 1;PEN 1;  0.25000!  0.25000; )\endinput

